Dimensional Analysis in Statistical Modelling

Building on recent work in statistical science, the paper presents a theory for modelling natural phenomena that unifies physical and statistical paradigms based on the underlying principle that a model must be nondimensionalizable. After all, such phenomena cannot depend on how the experimenter chooses to assess them. Yet the model itself must be comprised of quantities that can be determined theoretically or empirically. Hence, the underlying principle requires that the model represents these natural processes correctly no matter what scales and units of measurement are selected. This goal was realized for physical modelling through the celebrated theories of Buckingham and Bridgman and for statistical modellers through the invariance principle of Hunt and Stein. Building on recent research in statistical science, the paper shows how the latter can embrace and extend the former. The invariance principle is extended to encompass the Bayesian paradigm, thereby enabling an assessment of model uncertainty. The paper covers topics not ordinarily seen in statistical science regarding dimensions, scales, and units of quantities in statistical modelling. It shows the special difficulties that can arise when models involve transcendental functions, such as the logarithm which is used e.g. in likelihood analysis and is a singularity in the family of Box-Cox family of transformations. Further, it demonstrates the importance of the scale of measurement, in particular how differently modellers must handle ratio- and interval-scales

==> bib_frontmatter_to-do-list/commands_jz.tex <==




\RequirePackage[OT1]{fontenc}
\usepackage{amsthm,amsmath,natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% settings
%\pubyear{2005}
%\volume{0}
%\issue{0}
%\firstpage{1}
%\lastpage{8}

\startlocaldefs
\numberwithin{equation}{section}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\endlocaldefs


%%%%%%%%%%HARRY'S STUFF
%%%%%%%%%%%%
\usepackage{mathtools,amsmath,physics,framed,enumitem}
\usepackage{arydshln}
\usepackage{graphicx,float}
\usepackage{xcolor}
\usepackage{soul}
\usepackage{comment}
\usepackage{natbib,url}
\usepackage{bm}
\newcommand{\distas}[1]{\mathbin{\overset{#1}{\kern\z@\sim}}}%
\newcommand{\tbf}[1]{\textbf{#1}}%
\newcommand{\X}{\textbf{X}}%
\newcommand{\Y}{\textbf{Y}}%
\newcommand{\Cal}[1]{{\cal{#1}}}
\newcommand{\vvec}{\mbox{vec}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\Exp}{\mbox{Exp}}
\newcommand{\simd}{\stackrel{d}{\sim}}
\newcommand{\TRANSPOSE}{^\mathrm{T}}
\newcommand{\MAT}[1]{\textbf{#1}}%
\renewcommand{\a}{\alpha}%
\newcommand{\indep}{\raisebox{0.05em}{\rotatebox[origin=c]{90}{$\models$}}}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=red
}

\newsavebox{\mybox}\newsavebox{\mysim}
%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\usepackage{
amsmath, 
amsthm ,
amssymb, 
}
\theoremstyle{definition}
%\include{commands/commandsRev01_20140910}
\usepackage{fixltx2e,fix-cm}
\usepackage{graphicx}
\usepackage{multicol}
\usepackage{bm}
\usepackage{mathptmx} %uses times font


%\usepackage[backend=bibtex]{biblatex}
 \usepackage{natbib}
\usepackage{showidx}
\tolerance = 5000
\frenchspacing
%\PassOptionsToPackage{cmyk}{xcolor}
%\usepackage[notcite]{showkeys}

\usepackage{color}

%\usepackage{todonotes}

\usepackage{changepage}
\usepackage{subfig}   % for the adjustwidth environment


%\usepackage{index}
%%\usepackage{multind}
%%\usepackage{authorindex}
\usepackage[english]{babel}
\usepackage[T1]{fontenc}
\usepackage[ansinew]{inputenc}
%\usepackage[hyperindex=true]{hyperref}
\usepackage{makeidx}
%\makeindex




% et al
%\renewcommand{\BOthers}[1]{et al.\hbox{}}

%\usepackage{exercise}


%\usepackage{natbib}


%% To compile the author index you need to go to the 
%% terminal window command line and use
%%Use TexShop not Latexian
%%cd /Users/james/Dropbox/BOOK_STEPI_Feb1
%% makeindex -o ShaddickZidekSTEPI_20150224_GS.and ShaddickZidekSTEPI_20150224_GS.adx
\makeindex 


%%\makeindex{author}
\newcommand{\ina}[1]{\index{author}{#1}}
%%\makeindex{subject}
\newcommand{\ins}[1]{\index{subject}{#1}}



\definecolor{gray}{rgb}{0.95,0.95,0.95}
\definecolor{brightskyblue}{rgb}{0.9, 0.95, 0.99}

%%\usepackage{amsmath,array,graphics,verbatim,rotating,epsfig,graphicx}
%%\usepackage{makeidx} %If you want to generate an index, automatically
%%%%%%%%%%
%Page measurements

% \setlength{\parindent}{0cm}
% \setlength{\textheight}{23cm}
% \setlength{\textwidth}{15cm}
% \setlength{\oddsidemargin}{0cm}
% \setlength{\evensidemargin}{0cm}
% \addtolength{\topmargin}{-2cm}
% \setlength{\parskip}{0.3cm}

%Counters and Default Styles
 %%\setcounter{secnumdepth}{3}
 %%\setcounter{tocdepth}{3}


%%  NANCY ADDED%%%%%%%%%%%
\newcommand{\DA}{dimensional analysis}
\newcommand{\IP}{invariance principle}
\newcommand{\DHo}{dimensional homogeneity}
%\newcommand{\Re}{\mathbb{R}}

\newcommand{\Real}{{\rm I\!R}}

\usepackage[normalem]{ulem}   %% this gives \sout for strikethrough (not for math mode though)

%%%%%%%%%%%%%%%%

% Abbreviations
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\Cov}{\textrm{Cov}}
\newcommand{\mean}{\mathrm{mean}}
\newcommand{\se}{\mathrm{s.e.}}
\newcommand{\sd}{\mathrm{sd}}
\newcommand{\ie}{i.e.\ }
\newcommand{\iid}{\ensuremath{i.i.d.}}
\newcommand{\SE}{\mathrm{SE}}
\renewcommand{\vec}[1]{\mbox{\boldmath$#1$}}

\newcommand{\expec}[1]{\ensuremath{\mathbb{E}[#1]}}
%\newcommand{\var}[1]{\ensuremath{\mathrm{Var}[#1]}}
%\newcommand{\cov}[1]{\ensuremath{\mathrm{Cov}[#1]}}
\newcommand{\bd}[1]{\ensuremath{\mbox{\boldmath $#1$}}}
\newcommand{\corr}[1]{\ensuremath{\mathrm{Corr}[#1]}}



% useful shortcuts
\newcommand{\ones}[1]{\bf{1_{#1}}}
\newcommand{\zeros}[1]{\ensuremath{\mathbf{0_{#1}}}}
\newcommand{\half}{\scriptscriptstyle 1/2}
\newcommand{\hhalf}{{\ensuremath{\frac{1}{2}}}}
\newcommand{\overtwo}[1]{\ensuremath{{\frac{#1}{2}}}}
\newcommand{\sumi}{\ensuremath{\sum_{i=1}^{n}}}
\newcommand{\sumj}{\ensuremath{\sum_{j=1}^{m}}}


%Xs and Ys
\renewcommand{\Xi}{\ensuremath{X_i}}
\newcommand{\Yi}{\ensuremath{Y_i}}
\newcommand{\Zi}{\ensuremath{Z_i}}
\newcommand{\Xj}{\ensuremath{X_j}}
\newcommand{\Yj}{\ensuremath{Y_j}}
\newcommand{\Zj}{\ensuremath{Z_j}}
\newcommand{\Xij}{\ensuremath{X_{ij}}}
\newcommand{\Yij}{\ensuremath{Y_{ij}}}
\newcommand{\Zij}{\ensuremath{Z_{ij}}}

\newcommand{\Zbar}{\ensuremath{\bar{Z}}}
\newcommand{\Xbar}{\ensuremath{\bar{X}}}
\newcommand{\Ybar}{\ensuremath{\bar{Y}}}
\newcommand{\ybar}{\ensuremath{\bar{y}}}
\newcommand{\xbar}{\ensuremath{\bar{x}}}
\newcommand{\zbar}{\ensuremath{\bar{z}}}

\newcommand{\bfx}{\ensuremath{\mathbf{x}}}
\newcommand{\bfy}{\ensuremath{\mathbf{y}}}
\newcommand{\bfz}{\ensuremath{\mathbf{z}}}
\newcommand{\bfX}{\ensuremath{\mathbf{X}}}
\newcommand{\bfY}{\ensuremath{\mathbf{Y}}}
\newcommand{\bfZ}{\ensuremath{\mathbf{Z}}}


%\newcommand{\bfx}{\ensuremath{\mathbf{x}}}
%\newcommand{\bfy}{\ensuremath{\mathbf{y}}}
%\newcommand{\bfz}{\ensuremath{\mathbf{z}}}
%\newcommand{\bfX}{\ensuremath{\mathbf{X}}}
%\newcommand{\bfY}{\ensuremath{\mathbf{Y}}}
%\newcommand{\bfZ}{\ensuremath{\mathbf{Z}}}
\newcommand{\Sx}{S_{1\textbf{x}_1}}
\newcommand{\Sy}{S_{1\textbf{y}_1}}
\newcommand{\Sxinv}{S_{1\textbf{x}_1}^{-1}}
\newcommand{\Syinv}{S_{1\textbf{y}_1}^{-1}}
\newcommand{\Qx}{Q_{1\textbf{x}_1}}
\newcommand{\Qy}{Q_{1\textbf{y}_1}}

%Greek bold
\newcommand{\bfmu}{\ensuremath{\mathbf{\mu}}}
\newcommand{\bftheta}{\ensuremath{\mathbf{\theta}}}
\newcommand{\bfphi}{\ensuremath{\mathbf{\phi}}}
\newcommand{\bfbeta}{\ensuremath{\mathbf{\beta}}}
\newcommand{\bfepsilon}{\ensuremath{\mathbf{\epsilon}}}

%Tables
% c,r,l but with maths formatting
%%%%%%%%Change here
%%%%%%%%%%%%%%%%%%%%
%%\newcolumntype{C}{>{$}c<{$}}
%%\newcolumntype{R}{>{$}r<{$}}
%%\newcolumntype{L}{>{$}l<{$}}

%Special
\newcommand{\Sxx}{\ensuremath{S_{xx}}}
\newcommand{\app}{\mathrm{approx}}
\newcommand{\SMR}{\mathrm{SMR}}
\newcommand{\PPV}{\mathrm{PPV}}
\newcommand{\NPV}{\mathrm{NPV}}
\newcommand{\sens}{\mathrm{Se}}
\newcommand{\spec}{\mathrm{Sp}}
\newcommand{\prev}{p}
\newcommand{\RR}{\mathrm{RR}}
\newcommand{\AR}{\mathrm{AR}}
\newcommand{\OR}{\mathrm{OR}}
\newcommand{\paired}{\mathrm{paired}}
\newcommand{\nE}{\ensuremath{\bar{E}}}
\newcommand{\nD}{\ensuremath{\bar{D}}}
\newcommand{\nT}{\ensuremath{\bar{T}}}
\renewcommand{\strut}{\rule[-2mm]{0cm}{6mm}}
\newcommand{\MH}{\mathrm{MH}}
%\newcommand{\underset}[2]{nrel@{#2}%
 %   \binrel@@{\mathop{\kern\z@#2}\limits_{#1}}}


% Environments
\newenvironment{centre}{\begin{center}}{\end{center}}
\newenvironment{itemise}{\begin{itemize}}{\end{itemize}}

\newcommand{\ruth}[1]{\emph{\scshape #1}}
\newcommand{\OH}[1]{{\scshape #1}}




%Page measurements

%% \setlength{\parindent}{0cm}
% \setlength{\textheight}{25cm}
% \setlength{\textwidth}{17cm}
% \setlength{\oddsidemargin}{-1cm}
% \setlength{\evensidemargin}{-1cm}
% \addtolength{\topmargin}{-2cm}
% \setlength{\parskip}{0.5cm}

%Counters and Default Styles
 \setcounter{secnumdepth}{3}
 \setcounter{tocdepth}{3}


% Distributions

\newcommand{\Po}{\mbox{Po}}
\newcommand{\Bin}{\mbox{Bin}}
\newcommand{\Bern}{\mbox{Bern}}
\newcommand{\Beta}{\mbox{Beta}}
\newcommand{\Ga}{\mbox{Gamma}}
\newcommand{\InvChi}[1]{\mbox{Inv-}\chisq{#1}}
\newcommand{\InvGa}{\mbox{Inv-gamma}}
\newcommand{\Wishart}{\mbox{Wishart}}
\newcommand{\BetaBin}{\mbox{Beta-bin}}
\newcommand{\Mult}{\mbox{Multinomial}}
\newcommand{\Hypergeo}{\mbox{Hyper-geo}}
\newcommand{\Geo}{\mbox{Geo}}
\newcommand{\NegBin}{\mbox{Neg-bin}}
\newcommand{\Par}{\ensuremath{\textrm{Pareto}}}
\newcommand{\Maxwell}{\ensuremath{\textrm{Maxwell}}}
\newcommand{\Rayleigh}{\ensuremath{\textrm{Rayleigh}}}
\newcommand{\Dirich}{\ensuremath{\textrm{Dirichlet}}}
\newcommand{\LNorm}{\mathrm{LogNormal}}


%%indices


%%Definitions

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\i{\item}
\def\bdesc{\begin{description}}
\def\edesc{\end{description}}
\def\benum{\begin{enumerate}}
\def\eenum{\end{enumerate}}




% Abbreviations

%\newcommand{\mode}{\mathrm{mode}}
\newcommand{\novertwo}{\ensuremath{\scriptscriptstyle n/2}}

\newcommand{\prodi}{\ensuremath{\prod_{i=1}^{n}}}

\renewcommand{\Xi}{\ensuremath{X_i}}
\newcommand{\yi}{\ensuremath{y_i}}

\newcommand{\bft}{\ensuremath{\mathbf{t}}}
\newcommand{\bfT}{\ensuremath{\mathbf{T}}}
\newcommand{\bfu}{\ensuremath{\mathbf{u}}}
\newcommand{\bfm}{\ensuremath{\mathbf{m}}}

\newcommand{\bfalpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bfgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bfSigma}{\mbox{\boldmath $\Sigma$}}

\newcommand{\bfmle}{\ensuremath{\widehat{\bftheta}}}
\newcommand{\mle}{\ensuremath{\widehat{\theta}}}
\newcommand{\mode}{\ensuremath{\widetilde{\theta}}}
\newcommand{\bfmode}{\ensuremath{\widetilde{\bftheta}}}
\newcommand{\bfP}{\textbf{P}}
\newcommand{\bfQ}{\textbf{Q}}
\newcommand{\bfR}{\textbf{R}}
\newcommand{\bfS}{\textbf{S}}

%colors
%%\newrgbcolor{medgreen}{0.00 0.50 0.25}
%%\newrgbcolor{darkblue}{0.00 0.00 1.00}
%%\newrgbcolor{darkred}{1.00 0.00 0.00}
%%\newrgbcolor{darkredblue}{1.00 0.00 0.50}
%%\newrgbcolor{medgreenblue}{0.00 0.25 0.50}



% general

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{remarks}{Remarks}


%\newenvironment{example}[1][]{{\bf \itshape Example #1:} \itshape }{\upshape}

%%
\newcommand{\starreditem}{\addtocounter{enumi}{1}\item[*\labelenumi]}
\newcommand{\starredsubitem}{\addtocounter{enumii}{1}\item[*\labelenumii]}

\renewcommand{\paragraph}[1]{\vspace{.5cm}{\normalfont\normalsize\bfseries\emph{#1}}}



%%%%Greek letters
\def\ga{\gamma}
\newcommand{\de}{\delta}
%%\newcommand{\Ga}{\mbox{$\Gamma$}}
\def\al{\alpha}
\def\ep{\epsilon}
\def\ss{\sigma^2}
\def\ics{\chi^{-2}}
\def\ga{\gamma}
\def\B{\mbox{\boldmath$\beta$}}


%%%%%Bold versions
\def\B{\mbox{\boldmath$\beta$}}
\def\Si{\mbox{\boldmath$\Sigma$}}


%%%%%%Math symbols
\def\one{\mbox{\bf 1}}
%\def\B#1{\mbox{\boldmath $#1$}}
%need a pair of $'s for\def\iw{{\c\def\n{{\cal N}}
\def\iv{^{-1}}
\def\etr{\mbox{\rm etr}}
\def\tr{\mbox{\rm tr}}
\def\pp{^{(p)}}
\def\h{{\cal H}}
\def\iv{^{-1}}
\def\etr{\mbox{\rm etr}}
\def\tr{\mbox{\rm tr}}
\def\l({\left(}
\def\r){\right)}
\def\l{\left}


%%%%%%Other symbols
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\i{\item}



%%% Renewcommands
\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
%\newcommand{\tB}{\mbox{$\tilde{B}$}}
%\newcommand{\hB}{\mbox{$\hat{B}$}}
%\newcommand{\th}{\mbox{$\theta$}}

%%%Define new commands
%%
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\dred}{\textcolor{dred}}
\newcommand{\dblue}{\textcolor{dblue}}
\newcommand{\dgreen}{\textcolor{dgreen}}


\newcommand{\bb}{\bf{\beta}}
\newcommand{\bbeta}{\mathbf{\beta}}
\newcommand{\balpha}{\mathbf{\alpha}}

\newcommand{\N}{\mbox{N}}
\newcommand{\bmx}{\mathbf{x}}
\newcommand{\bmy}{\mathbf{y}}

\newcommand{\bgamma}{\mathbf{\gamma}}

\newcommand{\bmU}{\mathbf{U}}
\newcommand{\bmZ}{\mathbf{Z}}
\newcommand{\bmA}{\mathbf{A}}
\newcommand{\bmY}{\mathbf{Y}}


\newcommand{\bU}{\mathbf{U}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bmo}{\mathbf{-1}}
\newcommand{\bzero}{\mathbf{0}}

\newcommand{\bmR}{\mathbf{R}}


\newcommand{\bms}{\mathbf{s}}
\newcommand{\bmh}{\mathbf{h}}
\newcommand{\bmzero}{\mathbf{0}}

\newcommand{\bmt}{\mathbf{t}}
\newcommand{\bmd}{\mathbf{d}}
\newcommand{\bmmu}{\mathbf{\mu}}

 \newcommand{\bmV}{\mathbf{V}}

\newcommand{\bmI}{\mathbf{l}}


\newcommand{\bepsilon}{\mathbf{\epsilon}}

\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}

\newcommand{\bmz}{\mathbf{x}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bR}{\mathbf{R}}


\newcommand{\E}{\mbox{E}}
%\newcommand{\var}{\mbox{var}}
\newcommand{\by}{\mbox{by}}

\newcommand{\V}{\mbox{V}}
\newcommand{\C}{\mbox{COV}}


\newcommand{\tB}{\mbox{$\tilde{B}$}}
\newcommand{\hB}{\mbox{$\hat{B}$}}


\newenvironment{myenv}{\begin{adjustwidth}{0.75cm}{0.25cm}}{\end{adjustwidth}}



\newcommand{\bexmp}{\vspace{0.25cm}\begin{myenv}\begin{exmp}}
\newcommand{\eexmp}{\end{exmp}\end{myenv}\vspace{0.25cm}}

\newcommand\Index[1]{#1\index{#1}}

\newcommand\ext[2]{ {\em  #1 \vspace{0.1cm}}  \hfill  \break   \label{example:#2}}

\newcommand{\exsp}{\vspace{0.1cm}}
%%%%%%%%%%%%%%%%





==> bib_frontmatter_to-do-list/front_technicalstuff.tex <==
\RequirePackage[OT1]{fontenc}
\usepackage{amsthm,amsmath,natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

%settings
\pubyear{2020}
\volume{0}
\issue{0}
\firstpage{1}
\lastpage{48}

\startlocaldefs
\numberwithin{equation}{section}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\endlocaldefs

%% nancy added - to have example numbers remain same when "continuing"
\usepackage{thmtools}
% \renewcommand{\thmcontinues}[1]{continued}


%%%%%%%%%%HARRY'S STUFF
%%%%%%%%%%%%
\usepackage{mathtools,amsmath,physics,framed,enumitem}
\usepackage{arydshln}
\usepackage{graphicx,float}
\usepackage{xcolor}
\usepackage{soul}
\usepackage{comment}
\usepackage{natbib}
\usepackage{url}
\usepackage{bm}
\newcommand{\distas}[1]{\mathbin{\overset{#1}{\kern\z@\sim}}}%
\newcommand{\tbf}[1]{\textbf{#1}}%
\newcommand{\X}{\textbf{X}}%
\newcommand{\Y}{\textbf{Y}}%
\newcommand{\Cal}[1]{{\cal{#1}}}
\newcommand{\vvec}{\mbox{vec}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\Exp}{\mbox{Exp}}
\newcommand{\simd}{\stackrel{d}{\sim}}
\newcommand{\TRANSPOSE}{^\mathrm{T}}
\newcommand{\MAT}[1]{\textbf{#1}}%
\renewcommand{\a}{\alpha}%
\newcommand{\indep}{\raisebox{0.05em}{\rotatebox[origin=c]{90}{$\models$}}}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=red
}

\newsavebox{\mybox}\newsavebox{\mysim}
%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\usepackage{
amsmath, 
amsthm ,
amssymb, 
}
\theoremstyle{definition}
%\include{commands/commandsRev01_20140910}
\usepackage{fixltx2e,fix-cm}
\usepackage{graphicx}
\usepackage{multicol}
\usepackage{bm}
\usepackage{mathptmx} %uses times font


%\usepackage[backend=bibtex]{biblatex}
 \usepackage{natbib}
\usepackage{showidx}
\tolerance = 5000
\frenchspacing
%\PassOptionsToPackage{cmyk}{xcolor}
%\usepackage[notcite]{showkeys}

\usepackage{color}

%\usepackage{todonotes}

\usepackage{changepage}
\usepackage{subfig}   % for the adjustwidth environment


%\usepackage{index}
%%\usepackage{multind}
%%\usepackage{authorindex}
\usepackage[english]{babel}
\usepackage[T1]{fontenc}
\usepackage[ansinew]{inputenc}
%\usepackage[hyperindex=true]{hyperref}
\usepackage{makeidx}
%\makeindex




% et al
%\renewcommand{\BOthers}[1]{et al.\hbox{}}

%\usepackage{exercise}


%\usepackage{natbib}


%% To compile the author index you need to go to the 
%% terminal window command line and use
%%Use TexShop not Latexian
%%cd /Users/james/Dropbox/BOOK_STEPI_Feb1
%% makeindex -o ShaddickZidekSTEPI_20150224_GS.and ShaddickZidekSTEPI_20150224_GS.adx
\makeindex 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\makeindex{author}
%\newcommand{\ina}[1]{\index{author}{#1}}
%%\makeindex{subject}
%\newcommand{\ins}[1]{\index{subject}{#1}}



\definecolor{gray}{rgb}{0.95,0.95,0.95}
\definecolor{brightskyblue}{rgb}{0.9, 0.95, 0.99}

%%\usepackage{amsmath,array,graphics,verbatim,rotating,epsfig,graphicx}
%%\usepackage{makeidx} %If you want to generate an index, automatically
%%%%%%%%%%
%Page measurements

% \setlength{\parindent}{0cm}
% \setlength{\textheight}{23cm}
% \setlength{\textwidth}{15cm}
% \setlength{\oddsidemargin}{0cm}
% \setlength{\evensidemargin}{0cm}
% \addtolength{\topmargin}{-2cm}
% \setlength{\parskip}{0.3cm}

%Counters and Default Styles
 %%\setcounter{secnumdepth}{3}
 %%\setcounter{tocdepth}{3}


%%  NANCY ADDED%%%%%%%%%%%
\newcommand{\DA}{dimensional analysis}
\newcommand{\IP}{invariance principle}
\newcommand{\DHo}{dimensional homogeneity}
%\newcommand{\Re}{\mathbb{R}}

\newcommand{\Real}{{\rm I\!R}}

\usepackage[normalem]{ulem}   %% this gives \sout for strikethrough (not for math mode though)

%%%%%%%%%%%%%%%%

% Abbreviations
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\Cov}{\textrm{Cov}}
\newcommand{\mean}{\mathrm{mean}}
\newcommand{\se}{\mathrm{s.e.}}
\newcommand{\sd}{\mathrm{sd}}
\newcommand{\ie}{i.e.\ }
\newcommand{\iid}{\ensuremath{i.i.d.}}
\newcommand{\SE}{\mathrm{SE}}
\renewcommand{\vec}[1]{\mbox{\boldmath$#1$}}

\newcommand{\expec}[1]{\ensuremath{\mathbb{E}[#1]}}
%\newcommand{\var}[1]{\ensuremath{\mathrm{Var}[#1]}}
%\newcommand{\cov}[1]{\ensuremath{\mathrm{Cov}[#1]}}
\newcommand{\bd}[1]{\ensuremath{\mbox{\boldmath $#1$}}}
\newcommand{\corr}[1]{\ensuremath{\mathrm{Corr}[#1]}}



% useful shortcuts
\newcommand{\ones}[1]{\bf{1_{#1}}}
\newcommand{\zeros}[1]{\ensuremath{\mathbf{0_{#1}}}}
\newcommand{\half}{\scriptscriptstyle 1/2}
\newcommand{\hhalf}{{\ensuremath{\frac{1}{2}}}}
\newcommand{\overtwo}[1]{\ensuremath{{\frac{#1}{2}}}}
\newcommand{\sumi}{\ensuremath{\sum_{i=1}^{n}}}
\newcommand{\sumj}{\ensuremath{\sum_{j=1}^{m}}}


%Xs and Ys
\renewcommand{\Xi}{\ensuremath{X_i}}
\newcommand{\Yi}{\ensuremath{Y_i}}
\newcommand{\Zi}{\ensuremath{Z_i}}
\newcommand{\Xj}{\ensuremath{X_j}}
\newcommand{\Yj}{\ensuremath{Y_j}}
\newcommand{\Zj}{\ensuremath{Z_j}}
\newcommand{\Xij}{\ensuremath{X_{ij}}}
\newcommand{\Yij}{\ensuremath{Y_{ij}}}
\newcommand{\Zij}{\ensuremath{Z_{ij}}}

\newcommand{\Zbar}{\ensuremath{\bar{Z}}}
\newcommand{\Xbar}{\ensuremath{\bar{X}}}
\newcommand{\Ybar}{\ensuremath{\bar{Y}}}
\newcommand{\ybar}{\ensuremath{\bar{y}}}
\newcommand{\xbar}{\ensuremath{\bar{x}}}
\newcommand{\zbar}{\ensuremath{\bar{z}}}

\newcommand{\bfx}{\ensuremath{\mathbf{x}}}
\newcommand{\bfy}{\ensuremath{\mathbf{y}}}
\newcommand{\bfz}{\ensuremath{\mathbf{z}}}
\newcommand{\bfX}{\ensuremath{\mathbf{X}}}
\newcommand{\bfY}{\ensuremath{\mathbf{Y}}}
\newcommand{\bfZ}{\ensuremath{\mathbf{Z}}}


%\newcommand{\bfx}{\ensuremath{\mathbf{x}}}
%\newcommand{\bfy}{\ensuremath{\mathbf{y}}}
%\newcommand{\bfz}{\ensuremath{\mathbf{z}}}
%\newcommand{\bfX}{\ensuremath{\mathbf{X}}}
%\newcommand{\bfY}{\ensuremath{\mathbf{Y}}}
%\newcommand{\bfZ}{\ensuremath{\mathbf{Z}}}
\newcommand{\Sx}{S_{1\textbf{x}_1}}
\newcommand{\Sy}{S_{1\textbf{y}_1}}
\newcommand{\Sxinv}{S_{1\textbf{x}_1}^{-1}}
\newcommand{\Syinv}{S_{1\textbf{y}_1}^{-1}}
\newcommand{\Qx}{Q_{1\textbf{x}_1}}
\newcommand{\Qy}{Q_{1\textbf{y}_1}}

%Greek bold
\newcommand{\bfmu}{\ensuremath{\mathbf{\mu}}}
\newcommand{\bftheta}{\ensuremath{\mathbf{\theta}}}
\newcommand{\bfphi}{\ensuremath{\mathbf{\phi}}}
\newcommand{\bfbeta}{\ensuremath{\mathbf{\beta}}}
\newcommand{\bfepsilon}{\ensuremath{\mathbf{\epsilon}}}

%Tables
% c,r,l but with maths formatting
%%%%%%%%Change here
%%%%%%%%%%%%%%%%%%%%
%%\newcolumntype{C}{>{$}c<{$}}
%%\newcolumntype{R}{>{$}r<{$}}
%%\newcolumntype{L}{>{$}l<{$}}

%Special
\newcommand{\Sxx}{\ensuremath{S_{xx}}}
\newcommand{\app}{\mathrm{approx}}
\newcommand{\SMR}{\mathrm{SMR}}
\newcommand{\PPV}{\mathrm{PPV}}
\newcommand{\NPV}{\mathrm{NPV}}
\newcommand{\sens}{\mathrm{Se}}
\newcommand{\spec}{\mathrm{Sp}}
\newcommand{\prev}{p}
\newcommand{\RR}{\mathrm{RR}}
\newcommand{\AR}{\mathrm{AR}}
\newcommand{\OR}{\mathrm{OR}}
\newcommand{\paired}{\mathrm{paired}}
\newcommand{\nE}{\ensuremath{\bar{E}}}
\newcommand{\nD}{\ensuremath{\bar{D}}}
\newcommand{\nT}{\ensuremath{\bar{T}}}
\renewcommand{\strut}{\rule[-2mm]{0cm}{6mm}}
\newcommand{\MH}{\mathrm{MH}}
%\newcommand{\underset}[2]{nrel@{#2}%
 %   \binrel@@{\mathop{\kern\z@#2}\limits_{#1}}}


% Environments
\newenvironment{centre}{\begin{center}}{\end{center}}
\newenvironment{itemise}{\begin{itemize}}{\end{itemize}}

\newcommand{\ruth}[1]{\emph{\scshape #1}}
\newcommand{\OH}[1]{{\scshape #1}}




%Page measurements

%% \setlength{\parindent}{0cm}
% \setlength{\textheight}{25cm}
% \setlength{\textwidth}{17cm}
% \setlength{\oddsidemargin}{-1cm}
% \setlength{\evensidemargin}{-1cm}
% \addtolength{\topmargin}{-2cm}
% \setlength{\parskip}{0.5cm}

%Counters and Default Styles
 \setcounter{secnumdepth}{3}
 \setcounter{tocdepth}{3}


% Distributions

\newcommand{\Po}{\mbox{Po}}
\newcommand{\Bin}{\mbox{Bin}}
\newcommand{\Bern}{\mbox{Bern}}
\newcommand{\Beta}{\mbox{Beta}}
\newcommand{\Ga}{\mbox{Gamma}}
\newcommand{\InvChi}[1]{\mbox{Inv-}\chisq{#1}}
\newcommand{\InvGa}{\mbox{Inv-gamma}}
\newcommand{\Wishart}{\mbox{Wishart}}
\newcommand{\BetaBin}{\mbox{Beta-bin}}
\newcommand{\Mult}{\mbox{Multinomial}}
\newcommand{\Hypergeo}{\mbox{Hyper-geo}}
\newcommand{\Geo}{\mbox{Geo}}
\newcommand{\NegBin}{\mbox{Neg-bin}}
\newcommand{\Par}{\ensuremath{\textrm{Pareto}}}
\newcommand{\Maxwell}{\ensuremath{\textrm{Maxwell}}}
\newcommand{\Rayleigh}{\ensuremath{\textrm{Rayleigh}}}
\newcommand{\Dirich}{\ensuremath{\textrm{Dirichlet}}}
\newcommand{\LNorm}{\mathrm{LogNormal}}


%%indices


%%Definitions

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\i{\item}
\def\bdesc{\begin{description}}
\def\edesc{\end{description}}
\def\benum{\begin{enumerate}}
\def\eenum{\end{enumerate}}




% Abbreviations

%\newcommand{\mode}{\mathrm{mode}}
\newcommand{\novertwo}{\ensuremath{\scriptscriptstyle n/2}}

\newcommand{\prodi}{\ensuremath{\prod_{i=1}^{n}}}

\renewcommand{\Xi}{\ensuremath{X_i}}
\newcommand{\yi}{\ensuremath{y_i}}

\newcommand{\bft}{\ensuremath{\mathbf{t}}}
\newcommand{\bfT}{\ensuremath{\mathbf{T}}}
\newcommand{\bfu}{\ensuremath{\mathbf{u}}}
\newcommand{\bfm}{\ensuremath{\mathbf{m}}}

\newcommand{\bfalpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bfgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bfSigma}{\mbox{\boldmath $\Sigma$}}

\newcommand{\bfmle}{\ensuremath{\widehat{\bftheta}}}
\newcommand{\mle}{\ensuremath{\widehat{\theta}}}
\newcommand{\mode}{\ensuremath{\widetilde{\theta}}}
\newcommand{\bfmode}{\ensuremath{\widetilde{\bftheta}}}
\newcommand{\bfP}{\textbf{P}}
\newcommand{\bfQ}{\textbf{Q}}
\newcommand{\bfR}{\textbf{R}}
\newcommand{\bfS}{\textbf{S}}

%colors
%%\newrgbcolor{medgreen}{0.00 0.50 0.25}
%%\newrgbcolor{darkblue}{0.00 0.00 1.00}
%%\newrgbcolor{darkred}{1.00 0.00 0.00}
%%\newrgbcolor{darkredblue}{1.00 0.00 0.50}
%%\newrgbcolor{medgreenblue}{0.00 0.25 0.50}



% general

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{remarks}{Remarks}


%\newenvironment{example}[1][]{{\bf \itshape Example #1:} \itshape }{\upshape}

%%
\newcommand{\starreditem}{\addtocounter{enumi}{1}\item[*\labelenumi]}
\newcommand{\starredsubitem}{\addtocounter{enumii}{1}\item[*\labelenumii]}

\renewcommand{\paragraph}[1]{\vspace{.5cm}{\normalfont\normalsize\bfseries\emph{#1}}}



%%%%Greek letters
\def\ga{\gamma}
\newcommand{\de}{\delta}
%%\newcommand{\Ga}{\mbox{$\Gamma$}}
\def\al{\alpha}
\def\ep{\epsilon}
\def\ss{\sigma^2}
\def\ics{\chi^{-2}}
\def\ga{\gamma}
\def\B{\mbox{\boldmath$\beta$}}


%%%%%Bold versions
\def\B{\mbox{\boldmath$\beta$}}
\def\Si{\mbox{\boldmath$\Sigma$}}


%%%%%%Math symbols
\def\one{\mbox{\bf 1}}
%\def\B#1{\mbox{\boldmath $#1$}}
%need a pair of $'s for\def\iw{{\c\def\n{{\cal N}}
\def\iv{^{-1}}
\def\etr{\mbox{\rm etr}}
\def\tr{\mbox{\rm tr}}
\def\pp{^{(p)}}
\def\h{{\cal H}}
\def\iv{^{-1}}
\def\etr{\mbox{\rm etr}}
\def\tr{\mbox{\rm tr}}
\def\l({\left(}
\def\r){\right)}
\def\l{\left}


%%%%%%Other symbols
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\i{\item}



%%% Renewcommands
\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
%\newcommand{\tB}{\mbox{$\tilde{B}$}}
%\newcommand{\hB}{\mbox{$\hat{B}$}}
%\newcommand{\th}{\mbox{$\theta$}}

%%%Define new commands
%%
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\dred}{\textcolor{dred}}
\newcommand{\dblue}{\textcolor{dblue}}
\newcommand{\dgreen}{\textcolor{dgreen}}


\newcommand{\bb}{\bf{\beta}}
\newcommand{\bbeta}{\mathbf{\beta}}
\newcommand{\balpha}{\mathbf{\alpha}}

\newcommand{\N}{\mbox{N}}
\newcommand{\bmx}{\mathbf{x}}
\newcommand{\bmy}{\mathbf{y}}

\newcommand{\bgamma}{\mathbf{\gamma}}

\newcommand{\bmU}{\mathbf{U}}
\newcommand{\bmZ}{\mathbf{Z}}
\newcommand{\bmA}{\mathbf{A}}
\newcommand{\bmY}{\mathbf{Y}}


\newcommand{\bU}{\mathbf{U}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bmo}{\mathbf{-1}}
\newcommand{\bzero}{\mathbf{0}}

\newcommand{\bmR}{\mathbf{R}}


\newcommand{\bms}{\mathbf{s}}
\newcommand{\bmh}{\mathbf{h}}
\newcommand{\bmzero}{\mathbf{0}}

\newcommand{\bmt}{\mathbf{t}}
\newcommand{\bmd}{\mathbf{d}}
\newcommand{\bmmu}{\mathbf{\mu}}

 \newcommand{\bmV}{\mathbf{V}}

\newcommand{\bmI}{\mathbf{l}}


\newcommand{\bepsilon}{\mathbf{\epsilon}}

\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}

\newcommand{\bmz}{\mathbf{x}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bR}{\mathbf{R}}


\newcommand{\E}{\mbox{E}}
%\newcommand{\var}{\mbox{var}}
\newcommand{\by}{\mbox{by}}

\newcommand{\V}{\mbox{V}}
\newcommand{\C}{\mbox{COV}}


\newcommand{\tB}{\mbox{$\tilde{B}$}}
\newcommand{\hB}{\mbox{$\hat{B}$}}


\newenvironment{myenv}{\begin{adjustwidth}{0.75cm}{0.25cm}}{\end{adjustwidth}}



\newcommand{\bexmp}{\vspace{0.25cm}\begin{myenv}\begin{exmp}}
\newcommand{\eexmp}{\end{exmp}\end{myenv}\vspace{0.25cm}}

\newcommand\Index[1]{#1\index{#1}}

\newcommand\ext[2]{ {\em  #1 \vspace{0.1cm}}  \hfill  \break   \label{example:#2}}

\newcommand{\exsp}{\vspace{0.1cm}}
%%%%%%%%%%%%%%%%





==> front_technicalstuff.tex <==
\RequirePackage[OT1]{fontenc}
\usepackage{amsthm,amsmath,natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

%settings
\pubyear{2020}
\volume{0}
\issue{0}
\firstpage{1}
\lastpage{48}

\startlocaldefs
\numberwithin{equation}{section}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\endlocaldefs

%% nancy added - to have example numbers remain same when "continuing"
\usepackage{thmtools}
% \renewcommand{\thmcontinues}[1]{continued}


%%%%%%%%%%HARRY'S STUFF
%%%%%%%%%%%%
\usepackage{mathtools,amsmath,physics,framed,enumitem}
\usepackage{arydshln}
\usepackage{graphicx,float}
\usepackage{xcolor}
\usepackage{soul}
\usepackage{comment}
\usepackage{natbib}
\usepackage{url}
\usepackage{bm}
\newcommand{\distas}[1]{\mathbin{\overset{#1}{\kern\z@\sim}}}%
\newcommand{\tbf}[1]{\textbf{#1}}%
\newcommand{\X}{\textbf{X}}%
\newcommand{\Y}{\textbf{Y}}%
\newcommand{\Cal}[1]{{\cal{#1}}}
\newcommand{\vvec}{\mbox{vec}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\Exp}{\mbox{Exp}}
\newcommand{\simd}{\stackrel{d}{\sim}}
\newcommand{\TRANSPOSE}{^\mathrm{T}}
\newcommand{\MAT}[1]{\textbf{#1}}%
\renewcommand{\a}{\alpha}%
\newcommand{\indep}{\raisebox{0.05em}{\rotatebox[origin=c]{90}{$\models$}}}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=red
}

\newsavebox{\mybox}\newsavebox{\mysim}
%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\usepackage{
amsmath, 
amsthm ,
amssymb, 
}
\theoremstyle{definition}
%\include{commands/commandsRev01_20140910}
\usepackage{fixltx2e,fix-cm}
\usepackage{graphicx}
\usepackage{multicol}
\usepackage{bm}
\usepackage{mathptmx} %uses times font


%\usepackage[backend=bibtex]{biblatex}
 \usepackage{natbib}
\usepackage{showidx}
\tolerance = 5000
\frenchspacing
%\PassOptionsToPackage{cmyk}{xcolor}
%\usepackage[notcite]{showkeys}

\usepackage{color}

%\usepackage{todonotes}

\usepackage{changepage}
\usepackage{subfig}   % for the adjustwidth environment


%\usepackage{index}
%%\usepackage{multind}
%%\usepackage{authorindex}
\usepackage[english]{babel}
\usepackage[T1]{fontenc}
\usepackage[ansinew]{inputenc}
%\usepackage[hyperindex=true]{hyperref}
\usepackage{makeidx}
%\makeindex




% et al
%\renewcommand{\BOthers}[1]{et al.\hbox{}}

%\usepackage{exercise}


%\usepackage{natbib}


%% To compile the author index you need to go to the 
%% terminal window command line and use
%%Use TexShop not Latexian
%%cd /Users/james/Dropbox/BOOK_STEPI_Feb1
%% makeindex -o ShaddickZidekSTEPI_20150224_GS.and ShaddickZidekSTEPI_20150224_GS.adx
\makeindex 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\makeindex{author}
%\newcommand{\ina}[1]{\index{author}{#1}}
%%\makeindex{subject}
%\newcommand{\ins}[1]{\index{subject}{#1}}



\definecolor{gray}{rgb}{0.95,0.95,0.95}
\definecolor{brightskyblue}{rgb}{0.9, 0.95, 0.99}

%%\usepackage{amsmath,array,graphics,verbatim,rotating,epsfig,graphicx}
%%\usepackage{makeidx} %If you want to generate an index, automatically
%%%%%%%%%%
%Page measurements

% \setlength{\parindent}{0cm}
% \setlength{\textheight}{23cm}
% \setlength{\textwidth}{15cm}
% \setlength{\oddsidemargin}{0cm}
% \setlength{\evensidemargin}{0cm}
% \addtolength{\topmargin}{-2cm}
% \setlength{\parskip}{0.3cm}

%Counters and Default Styles
 %%\setcounter{secnumdepth}{3}
 %%\setcounter{tocdepth}{3}


%%  NANCY ADDED%%%%%%%%%%%
\newcommand{\DA}{dimensional analysis}
\newcommand{\IP}{invariance principle}
\newcommand{\DHo}{dimensional homogeneity}
%\newcommand{\Re}{\mathbb{R}}

\newcommand{\Real}{{\rm I\!R}}

\usepackage[normalem]{ulem}   %% this gives \sout for strikethrough (not for math mode though)

%%%%%%%%%%%%%%%%

% Abbreviations
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\Cov}{\textrm{Cov}}
\newcommand{\mean}{\mathrm{mean}}
\newcommand{\se}{\mathrm{s.e.}}
\newcommand{\sd}{\mathrm{sd}}
\newcommand{\ie}{i.e.\ }
\newcommand{\iid}{\ensuremath{i.i.d.}}
\newcommand{\SE}{\mathrm{SE}}
\renewcommand{\vec}[1]{\mbox{\boldmath$#1$}}

\newcommand{\expec}[1]{\ensuremath{\mathbb{E}[#1]}}
%\newcommand{\var}[1]{\ensuremath{\mathrm{Var}[#1]}}
%\newcommand{\cov}[1]{\ensuremath{\mathrm{Cov}[#1]}}
\newcommand{\bd}[1]{\ensuremath{\mbox{\boldmath $#1$}}}
\newcommand{\corr}[1]{\ensuremath{\mathrm{Corr}[#1]}}



% useful shortcuts
\newcommand{\ones}[1]{\bf{1_{#1}}}
\newcommand{\zeros}[1]{\ensuremath{\mathbf{0_{#1}}}}
\newcommand{\half}{\scriptscriptstyle 1/2}
\newcommand{\hhalf}{{\ensuremath{\frac{1}{2}}}}
\newcommand{\overtwo}[1]{\ensuremath{{\frac{#1}{2}}}}
\newcommand{\sumi}{\ensuremath{\sum_{i=1}^{n}}}
\newcommand{\sumj}{\ensuremath{\sum_{j=1}^{m}}}


%Xs and Ys
\renewcommand{\Xi}{\ensuremath{X_i}}
\newcommand{\Yi}{\ensuremath{Y_i}}
\newcommand{\Zi}{\ensuremath{Z_i}}
\newcommand{\Xj}{\ensuremath{X_j}}
\newcommand{\Yj}{\ensuremath{Y_j}}
\newcommand{\Zj}{\ensuremath{Z_j}}
\newcommand{\Xij}{\ensuremath{X_{ij}}}
\newcommand{\Yij}{\ensuremath{Y_{ij}}}
\newcommand{\Zij}{\ensuremath{Z_{ij}}}

\newcommand{\Zbar}{\ensuremath{\bar{Z}}}
\newcommand{\Xbar}{\ensuremath{\bar{X}}}
\newcommand{\Ybar}{\ensuremath{\bar{Y}}}
\newcommand{\ybar}{\ensuremath{\bar{y}}}
\newcommand{\xbar}{\ensuremath{\bar{x}}}
\newcommand{\zbar}{\ensuremath{\bar{z}}}

\newcommand{\bfx}{\ensuremath{\mathbf{x}}}
\newcommand{\bfy}{\ensuremath{\mathbf{y}}}
\newcommand{\bfz}{\ensuremath{\mathbf{z}}}
\newcommand{\bfX}{\ensuremath{\mathbf{X}}}
\newcommand{\bfY}{\ensuremath{\mathbf{Y}}}
\newcommand{\bfZ}{\ensuremath{\mathbf{Z}}}


%\newcommand{\bfx}{\ensuremath{\mathbf{x}}}
%\newcommand{\bfy}{\ensuremath{\mathbf{y}}}
%\newcommand{\bfz}{\ensuremath{\mathbf{z}}}
%\newcommand{\bfX}{\ensuremath{\mathbf{X}}}
%\newcommand{\bfY}{\ensuremath{\mathbf{Y}}}
%\newcommand{\bfZ}{\ensuremath{\mathbf{Z}}}
\newcommand{\Sx}{S_{1\textbf{x}_1}}
\newcommand{\Sy}{S_{1\textbf{y}_1}}
\newcommand{\Sxinv}{S_{1\textbf{x}_1}^{-1}}
\newcommand{\Syinv}{S_{1\textbf{y}_1}^{-1}}
\newcommand{\Qx}{Q_{1\textbf{x}_1}}
\newcommand{\Qy}{Q_{1\textbf{y}_1}}

%Greek bold
\newcommand{\bfmu}{\ensuremath{\mathbf{\mu}}}
\newcommand{\bftheta}{\ensuremath{\mathbf{\theta}}}
\newcommand{\bfphi}{\ensuremath{\mathbf{\phi}}}
\newcommand{\bfbeta}{\ensuremath{\mathbf{\beta}}}
\newcommand{\bfepsilon}{\ensuremath{\mathbf{\epsilon}}}

%Tables
% c,r,l but with maths formatting
%%%%%%%%Change here
%%%%%%%%%%%%%%%%%%%%
%%\newcolumntype{C}{>{$}c<{$}}
%%\newcolumntype{R}{>{$}r<{$}}
%%\newcolumntype{L}{>{$}l<{$}}

%Special
\newcommand{\Sxx}{\ensuremath{S_{xx}}}
\newcommand{\app}{\mathrm{approx}}
\newcommand{\SMR}{\mathrm{SMR}}
\newcommand{\PPV}{\mathrm{PPV}}
\newcommand{\NPV}{\mathrm{NPV}}
\newcommand{\sens}{\mathrm{Se}}
\newcommand{\spec}{\mathrm{Sp}}
\newcommand{\prev}{p}
\newcommand{\RR}{\mathrm{RR}}
\newcommand{\AR}{\mathrm{AR}}
\newcommand{\OR}{\mathrm{OR}}
\newcommand{\paired}{\mathrm{paired}}
\newcommand{\nE}{\ensuremath{\bar{E}}}
\newcommand{\nD}{\ensuremath{\bar{D}}}
\newcommand{\nT}{\ensuremath{\bar{T}}}
\renewcommand{\strut}{\rule[-2mm]{0cm}{6mm}}
\newcommand{\MH}{\mathrm{MH}}
%\newcommand{\underset}[2]{nrel@{#2}%
 %   \binrel@@{\mathop{\kern\z@#2}\limits_{#1}}}


% Environments
\newenvironment{centre}{\begin{center}}{\end{center}}
\newenvironment{itemise}{\begin{itemize}}{\end{itemize}}

\newcommand{\ruth}[1]{\emph{\scshape #1}}
\newcommand{\OH}[1]{{\scshape #1}}




%Page measurements

%% \setlength{\parindent}{0cm}
% \setlength{\textheight}{25cm}
% \setlength{\textwidth}{17cm}
% \setlength{\oddsidemargin}{-1cm}
% \setlength{\evensidemargin}{-1cm}
% \addtolength{\topmargin}{-2cm}
% \setlength{\parskip}{0.5cm}

%Counters and Default Styles
 \setcounter{secnumdepth}{3}
 \setcounter{tocdepth}{3}


% Distributions

\newcommand{\Po}{\mbox{Po}}
\newcommand{\Bin}{\mbox{Bin}}
\newcommand{\Bern}{\mbox{Bern}}
\newcommand{\Beta}{\mbox{Beta}}
\newcommand{\Ga}{\mbox{Gamma}}
\newcommand{\InvChi}[1]{\mbox{Inv-}\chisq{#1}}
\newcommand{\InvGa}{\mbox{Inv-gamma}}
\newcommand{\Wishart}{\mbox{Wishart}}
\newcommand{\BetaBin}{\mbox{Beta-bin}}
\newcommand{\Mult}{\mbox{Multinomial}}
\newcommand{\Hypergeo}{\mbox{Hyper-geo}}
\newcommand{\Geo}{\mbox{Geo}}
\newcommand{\NegBin}{\mbox{Neg-bin}}
\newcommand{\Par}{\ensuremath{\textrm{Pareto}}}
\newcommand{\Maxwell}{\ensuremath{\textrm{Maxwell}}}
\newcommand{\Rayleigh}{\ensuremath{\textrm{Rayleigh}}}
\newcommand{\Dirich}{\ensuremath{\textrm{Dirichlet}}}
\newcommand{\LNorm}{\mathrm{LogNormal}}


%%indices


%%Definitions

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\i{\item}
\def\bdesc{\begin{description}}
\def\edesc{\end{description}}
\def\benum{\begin{enumerate}}
\def\eenum{\end{enumerate}}




% Abbreviations

%\newcommand{\mode}{\mathrm{mode}}
\newcommand{\novertwo}{\ensuremath{\scriptscriptstyle n/2}}

\newcommand{\prodi}{\ensuremath{\prod_{i=1}^{n}}}

\renewcommand{\Xi}{\ensuremath{X_i}}
\newcommand{\yi}{\ensuremath{y_i}}

\newcommand{\bft}{\ensuremath{\mathbf{t}}}
\newcommand{\bfT}{\ensuremath{\mathbf{T}}}
\newcommand{\bfu}{\ensuremath{\mathbf{u}}}
\newcommand{\bfm}{\ensuremath{\mathbf{m}}}

\newcommand{\bfalpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bfgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bfSigma}{\mbox{\boldmath $\Sigma$}}

\newcommand{\bfmle}{\ensuremath{\widehat{\bftheta}}}
\newcommand{\mle}{\ensuremath{\widehat{\theta}}}
\newcommand{\mode}{\ensuremath{\widetilde{\theta}}}
\newcommand{\bfmode}{\ensuremath{\widetilde{\bftheta}}}
\newcommand{\bfP}{\textbf{P}}
\newcommand{\bfQ}{\textbf{Q}}
\newcommand{\bfR}{\textbf{R}}
\newcommand{\bfS}{\textbf{S}}

%colors
%%\newrgbcolor{medgreen}{0.00 0.50 0.25}
%%\newrgbcolor{darkblue}{0.00 0.00 1.00}
%%\newrgbcolor{darkred}{1.00 0.00 0.00}
%%\newrgbcolor{darkredblue}{1.00 0.00 0.50}
%%\newrgbcolor{medgreenblue}{0.00 0.25 0.50}



% general

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{remarks}{Remarks}


%\newenvironment{example}[1][]{{\bf \itshape Example #1:} \itshape }{\upshape}

%%
\newcommand{\starreditem}{\addtocounter{enumi}{1}\item[*\labelenumi]}
\newcommand{\starredsubitem}{\addtocounter{enumii}{1}\item[*\labelenumii]}

\renewcommand{\paragraph}[1]{\vspace{.5cm}{\normalfont\normalsize\bfseries\emph{#1}}}



%%%%Greek letters
\def\ga{\gamma}
\newcommand{\de}{\delta}
%%\newcommand{\Ga}{\mbox{$\Gamma$}}
\def\al{\alpha}
\def\ep{\epsilon}
\def\ss{\sigma^2}
\def\ics{\chi^{-2}}
\def\ga{\gamma}
\def\B{\mbox{\boldmath$\beta$}}


%%%%%Bold versions
\def\B{\mbox{\boldmath$\beta$}}
\def\Si{\mbox{\boldmath$\Sigma$}}


%%%%%%Math symbols
\def\one{\mbox{\bf 1}}
%\def\B#1{\mbox{\boldmath $#1$}}
%need a pair of $'s for\def\iw{{\c\def\n{{\cal N}}
\def\iv{^{-1}}
\def\etr{\mbox{\rm etr}}
\def\tr{\mbox{\rm tr}}
\def\pp{^{(p)}}
\def\h{{\cal H}}
\def\iv{^{-1}}
\def\etr{\mbox{\rm etr}}
\def\tr{\mbox{\rm tr}}
\def\l({\left(}
\def\r){\right)}
\def\l{\left}


%%%%%%Other symbols
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\i{\item}



%%% Renewcommands
\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
%\newcommand{\tB}{\mbox{$\tilde{B}$}}
%\newcommand{\hB}{\mbox{$\hat{B}$}}
%\newcommand{\th}{\mbox{$\theta$}}

%%%Define new commands
%%
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\dred}{\textcolor{dred}}
\newcommand{\dblue}{\textcolor{dblue}}
\newcommand{\dgreen}{\textcolor{dgreen}}


\newcommand{\bb}{\bf{\beta}}
\newcommand{\bbeta}{\mathbf{\beta}}
\newcommand{\balpha}{\mathbf{\alpha}}

\newcommand{\N}{\mbox{N}}
\newcommand{\bmx}{\mathbf{x}}
\newcommand{\bmy}{\mathbf{y}}

\newcommand{\bgamma}{\mathbf{\gamma}}

\newcommand{\bmU}{\mathbf{U}}
\newcommand{\bmZ}{\mathbf{Z}}
\newcommand{\bmA}{\mathbf{A}}
\newcommand{\bmY}{\mathbf{Y}}


\newcommand{\bU}{\mathbf{U}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bmo}{\mathbf{-1}}
\newcommand{\bzero}{\mathbf{0}}

\newcommand{\bmR}{\mathbf{R}}


\newcommand{\bms}{\mathbf{s}}
\newcommand{\bmh}{\mathbf{h}}
\newcommand{\bmzero}{\mathbf{0}}

\newcommand{\bmt}{\mathbf{t}}
\newcommand{\bmd}{\mathbf{d}}
\newcommand{\bmmu}{\mathbf{\mu}}

 \newcommand{\bmV}{\mathbf{V}}

\newcommand{\bmI}{\mathbf{l}}


\newcommand{\bepsilon}{\mathbf{\epsilon}}

\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}

\newcommand{\bmz}{\mathbf{x}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bR}{\mathbf{R}}


\newcommand{\E}{\mbox{E}}
%\newcommand{\var}{\mbox{var}}
\newcommand{\by}{\mbox{by}}

\newcommand{\V}{\mbox{V}}
\newcommand{\C}{\mbox{COV}}


\newcommand{\tB}{\mbox{$\tilde{B}$}}
\newcommand{\hB}{\mbox{$\hat{B}$}}


\newenvironment{myenv}{\begin{adjustwidth}{0.75cm}{0.25cm}}{\end{adjustwidth}}



\newcommand{\bexmp}{\vspace{0.25cm}\begin{myenv}\begin{exmp}}
\newcommand{\eexmp}{\end{exmp}\end{myenv}\vspace{0.25cm}}

\newcommand\Index[1]{#1\index{#1}}

\newcommand\ext[2]{ {\em  #1 \vspace{0.1cm}}  \hfill  \break   \label{example:#2}}

\newcommand{\exsp}{\vspace{0.1cm}}
%%%%%%%%%%%%%%%%




